Learning Navigation Costs from Demonstration with Semantic Observations

This paper focuses on inverse reinforcement learning (IRL) for autonomous robot navigation using semantic observations. The objective is to infer a cost function that explains demonstrated behavior while relying only on the expert's observations and state-control trajectory. We develop a map encoder, which infers semantic class probabilities from the observation sequence, and a cost encoder, defined as deep neural network over the semantic features. Since the expert cost is not directly observable, the representation parameters can only be optimized by differentiating the error between demonstrated controls and a control policy computed from the cost estimate. The error is optimized using a closed-form subgradient computed only over a subset of promising states via a motion planning algorithm. We show that our approach learns to follow traffic rules in the autonomous driving CARLA simulator by relying on semantic observations of cars, sidewalks and road lanes.

==> tex/CostLearning.tex <==
\section{Cost Learning via Differentiable Planning}
\label{sec:cost_learning}

\begin{algorithm2e}[t]
\caption{Training: learn cost function parameters $\vec{\theta}$}
\label{alg:train}
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{Demonstrations $\mathcal{D} \!=\! \crl{(\vec{x}_{t,n},\vec{u}_{t,n}^*,
\vec{P}_{t,n}, \vec{x}_{g,n})}_{t=1, n=1}^{T_n,N}\!\!$}
\While{$\vec{\theta}$ not converged}{
  $\mathcal{L}(\vec{\theta}) \gets 0$\;
  \For{$n = 1, \ldots,N$ \textbf{and} $t = 1,\ldots, T_n$}{
    Update $c_{t,n}$ based on $\vec{x}_{t,n}$ and $\vec{P}_{t,n}$ as in 
    Sec.~\ref{sec:cost_representation}\;
    Obtain $Q_{t,n}^*(\vec{x},\vec{u})$ from DSP~\eqref{eqn:Q} with stage cost $c_{t,n}$\;
    Obtain $\pi_{t,n}(\vec{u} | \vec{x}_{t,n})$ from $Q_{t,n}^*(\vec{x}_{t,n},\vec{u})$ 
    via Eq.~\eqref{eq:stochastic_policy}\;
    $\mathcal{L}(\vec{\theta}) \gets \mathcal{L}(\vec{\theta}) -\log \pi_{t, n} 
    (\vec{u}_{t,n}^*|\vec{x}_{t,n})$\;
  }
  Update $\vec{\theta} \gets \vec{\theta} - \alpha \nabla \mathcal{L}(\vec{\theta})$ via Prop.~\ref{prop:chain_rule}\;
}
\Output{$\vec{\theta}$} 
\end{algorithm2e}

\begin{algorithm2e}[t]
\caption{Testing: compute control policy for learned $\vec{\theta}$}
\label{alg:test}
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

\Input{Start state $\vec{x}_s$, goal state $\vec{x}_g$, optimized $\vec{\theta}$}
Current state $\vec{x}_t \gets \vec{x}_s$\;
\While{$\vec{x}_t \neq \vec{x}_g$}{
  Make an observation $\vec{P}_t$\;
  Update $c_t$ based on $\vec{x}_t$ and $\vec{P}_t$ as in Sec.~\ref{sec:cost_representation}\;
  Obtain $\pi_t(\vec{u} | \vec{x}_t)$ from $Q_t^*(\vec{x}_t,\vec{u})$ via 
  Eq.~\eqref{eq:stochastic_policy}\;
  Update $\vec{x}_t \gets f(\vec{x}_t, \vec{u}_t)$ via $\vec{u}_t := 
  \argmax_{\vec{u}} \pi_t(\vec{u}|\vec{x}_t)$\;
}
\Output{Navigation succeeds or fails.}
\end{algorithm2e}

We focus on optimizing the parameters $\vec{\theta}$ of the cost representation 
$c_t(\vec{x},\vec{u} ; \vec{P}_{1:t}, \vec{\theta})$ developed in 
Sec.~\ref{sec:cost_representation}. 
Since the true cost $c^*$ is not directly observable, we need to 
differentiate the loss function $\mathcal{L}(\vec{\theta})$ in~\eqref{eq:loss}, 
which, in turn, requires differentiating through the DSP problem 
in~\eqref{eqn:Q} with respect to the cost function estimate $c_t$. 

Value Iteration Networks (VIN)~\citep{Tamar2016VIN} shows that $T$ iterations 
of the value iteration algorithm can be approximated by a neural network with 
$T$ convolutional and minpooling layers. 
This allows VIN to be differentiable with respect to the stage cost. 
While VIN can be modified to operate with a finite horizon and produce a 
non-stationary policy, it would still be based on full Bellman backups 
(convolutions and min-pooling) over the entire state space. 
As a result, VIN scales poorly with the state-space size, while it might 
not even be necessary to determine the optimal cost-to-go $Q_t^*(\vec{x},\vec{u})$ 
at every state $\vec{x} \in \mathcal{X}$ and control $\vec{u} \in \mathcal{U}$ 
in the case of partially observable environments.

Instead of using dynamic programming to solve the DSP~\eqref{eqn:Q}, 
any motion planning algorithm (e.g., A*~\citep{Hart1968Astar, ARA},
RRT~\citep{Lavalle1998RRT, Karaman2011RRTstar}, etc.) that returns the optimal
cost-to-go $Q_t^*(\vec{x},\vec{u})$ over a subset of the state-control space provides
an accurate enough solution.
For example, a backwards A* search applied to problem~\eqref{eqn:Q} with 
start state $\vec{x}_g$, goal state $\vec{x} \in \mathcal{X}$, 
and predecessors expansions according to the motion model $f$ provides 
an upper bound to the optimal cost-to-go:
\begin{equation*}
%\label{eqn:overestimate}
\begin{aligned}
Q_t^*(\vec{x},\vec{u}) &= 
c_t(\vec{x},\vec{u}) + g(f(\vec{x},\vec{u})) \; &\forall f(\vec{x},\vec{u}) 
&\in \text{CLOSED},\\
Q_t^*(\vec{x},\vec{u}) &\leq 
c_t(\vec{x},\vec{u}) + g(f(\vec{x},\vec{u})) \; &\forall f(\vec{x},\vec{u}) 
&\not\in \text{CLOSED},
\end{aligned}
\end{equation*}
where $g$ are the values computed by A* for expanded nodes in the CLOSED list 
and visited nodes in the OPEN list. 
Thus, a Boltzmann policy $\pi_t(\vec{u} \mid \vec{x})$ can be defined using the 
$g$-values returned by A* for all 
$\vec{x} \in \text{CLOSED} \cup \text{OPEN} \subseteq \mathcal{X}$ and a uniform distribution 
over $\mathcal{U}$ for all other states $\vec{x}$. 
A* would significantly improves the efficiency of VIN or other full backup 
Dynamic Programming variants by performing local Bellman backups on promising 
states (the CLOSED list).

In addition to improving the efficiency of the forward computation of 
$Q_t^*(\vec{x},\vec{u})$, using a planning algorithm to solve~\eqref{eqn:Q} is also more 
efficient in back-propagating errors with respect to $\vec{\theta}$. 
In detail, using the subgradient method~\cite{Shor2012Subgradient,Ratliff2006MMP} to 
optimize $\mathcal{L}(\vec{\theta})$ leads to a closed-form (sub)gradient of 
$Q_t^*(\vec{x}_t,\vec{u}_t)$ with respect to $c_t(\vec{x},\vec{u})$, 
removing the need for back-propagation through multiple convolutional or min-pooling layers. 
We proceed by rewriting $Q_t^*(\vec{x}_t,\vec{u}_t)$ in a form that makes its subgradient 
with respect to $c_t(\vec{x},\vec{u})$ obvious. 
Let $\mathcal{T}(\vec{x}_t,\vec{u}_t)$ be the set of feasible state-control trajectories 
$\vec{\tau} \defeq \vec{x}_t,\vec{u}_t,\vec{x}_{t+1},\vec{u}_{t+1},\ldots,\vec{x}_{T-1},
\vec{u}_{T-1}$ starting at $\vec{x}_t$, $\vec{u}_t$ and satisfying $\vec{x}_{k+1} = 
f(\vec{x}_k,\vec{u}_k)$ for $k = t,\ldots,T-1$ with $\vec{x}_g = \vec{x}_T$. 
Let $\vec{\tau}^* \in \mathcal{T}(\vec{x}_t,\vec{u}_t)$ be an optimal trajectory 
corresponding to the optimal cost-to-go function $Q^*_t(\vec{x}_t,\vec{u}_t)$ of a 
deterministic shortest path problem, i.e., the controls in $\vec{\tau}^*$ satisfy 
the additional constraint $\vec{u}_{k} = \arg\min_{\vec{u} \in \mathcal{U}} 
Q^*_t(\vec{x}_{k},\vec{u})$ for $k = t+1,\ldots,T-1$. 
Let $\mu_{\vec{\tau}}(\vec{x},\vec{u}) \defeq \sum_{k=t}^{T-1} 
\indicator_{(\vec{x}_k,\vec{u}_k) = (\vec{x},\vec{u})}$ be a state-control visitation 
function indicating if $(\vec{x},\vec{u})$ is visited by $\vec{\tau}$. 
With these definitions, we can view the optimal cost-to-go function 
$Q^*_t(\vec{x}_t,\vec{u}_t)$ as minimum over $\mathcal{T}(\vec{x}_t,\vec{u}_t)$ of 
the inner product of the cost function $c_t$ and the visitation function $\mu_{\vec{\tau}}$:
\begin{equation}
\label{eq:inner_product_q}
Q^*_t(\vec{x}_t,\vec{u}_t) = \argmin_{\vec{\tau} \in \mathcal{T}(\vec{x}_t,\vec{u}_t)}  
\sum_{\vec{x} \in \mathcal{X},\vec{u}\in\mathcal{U}} c_t(\vec{x},\vec{u}) 
\mu_{\vec{\tau}}(\vec{x},\vec{u})
\end{equation}
where $\mathcal{X}$ can be assumed finite because both $T$ and $\mathcal{U}$ are finite. 
This form allows us to (sub)differentiate $Q^*_t(\vec{x}_t,\vec{u}_t)$ with respect to 
$c_t(\vec{x},\vec{u})$ for any $\vec{x} \in \mathcal{X}$, $\vec{u} \in \mathcal{U}$.

\begin{lemma}
\label{lemma:subgradient}
Let $f(\vec{x},\vec{y})$ be differentiable and convex in $\vec{x}$. 
Then, $\nabla_{\vec{x}} f(\vec{x}, \vec{y}^*)$, where $\vec{y}^* \defeq \arg\min_{\vec{y}} 
f(\vec{x},\vec{y})$, is a subgradient of the piecewise-differentiable 
convex function $g(\vec{x}) \defeq \min_{\vec{y}} f(\vec{x},\vec{y})$.
\end{lemma}

Applying Lemma~\ref{lemma:subgradient} to~\eqref{eq:inner_product_q} leads to the 
following subgradient of the optimal cost-to-go function:
\begin{equation}
\label{eq:subgradient_q}
\frac{\partial Q^*_t(\vec{x}_t,\vec{u}_t)}{\partial c_t(\vec{x},\vec{u})} = 
\mu_{\vec{\tau}^*}(\vec{x},\vec{u}),
\end{equation}
which can be obtained from the optimal trajectory $\vec{\tau}^*$ corresponding to 
$Q^*_t(\vec{x}_t,\vec{u}_t)$. 
This result and the chain rule allow us to obtain the complete (sub)gradient of 
$\mathcal{L}(\vec{\theta})$.

\begin{proposition}\footnote{Number here seems wrong. \TODO{It is because Lemma and Proposition are on the same counter in jmlrutils.sty. We might not have space to keep both anyways.}}
\label{prop:chain_rule}
A subgradient of the loss function $\mathcal{L}(\vec{\theta})$ in~\eqref{eq:loss} 
with respect to the cost function parameters $\vec{\theta}$ can be obtained as follows:
\begin{align}
&\frac{\partial \mathcal{L}(\vec{\theta})}{\partial \vec{\theta}} = 
- \sum_{n=1}^N \sum_{t=1}^{T_n} \frac{\partial \log \pi_{t,n}(\vec{u}_{t,n}^* 
\mid \vec{x}_{t,n})}{\partial \vec{\theta}}\\
&=- \sum_{n=1}^N \sum_{t=1}^{T_n}\sum_{\vec{u}_{t,n} \in \mathcal{U}} 
\frac{\partial \log \pi_{t,n}(\vec{u}_{t,n}^* \mid \vec{x}_{t,n})}
{\partial Q_{t,n}^*(\vec{x}_{t,n},\vec{u}_{t,n})} 
\frac{\partial Q_{t,n}^*(\vec{x}_{t,n},\vec{u}_{t,n})}
{\partial \vec{\theta}}\notag
\end{align}
where the first term has a closed-form, while the second term is available 
from~\eqref{eq:subgradient_q} and the cost representation in 
Sec.~\ref{sec:cost_representation}:
\begin{align}
&\frac{\partial \log \pi_{t,n}(\vec{u}_{t,n}^* \mid \vec{x}_{t,n})}
{\partial Q_{t,n}^*(\vec{x}_{t,n},\vec{u}_{t,n})} = 
\prl{\indicator_{\{\vec{u}_{t,n} = \vec{u}_{t,n}^*\}} - 
\pi_{t,n}(\vec{u}_{t,n} | \vec{x}_{t,n})}\notag\\
&\frac{\partial Q_{t,n}^*(\vec{x}_{t,n},\vec{u}_{t,n})}{\partial \vec{\theta}} = 
\!\!\!\!\!\sum_{(\vec{x},\vec{u}) \in \vec{\tau}^*} \!\!\!\!\!
\frac{\partial Q_{t,n}^*(\vec{x}_{t,n},\vec{u}_{t,n})}{\partial c_t(\vec{x},\vec{u})} 
\frac{\partial c_t(\vec{x},\vec{u})}{\partial \vec{\theta}}
\end{align}
\end{proposition}

The computation graph structure implied by Prop.~\ref{prop:chain_rule} is 
illustrated in Fig.~\ref{fig:approach}. 
The graph consists of a cost representation layer and a differentiable planning layer, 
allowing end-to-end minimization of $\mathcal{L}(\vec{\theta})$ via stochastic 
(sub)gradient descent. 
Full algorithms for the training and testing phases (Fig.~\ref{fig:approach}) are 
shown in Alg.~\ref{alg:train} and Alg.~\ref{alg:test} (\TODO{can we put two algorithms side by side}).

Although the form of the gradient in Prop.~\ref{prop:chain_rule} is similar to
that in~\citet{Ziebart2008MaxEnt}, our contributions are
orthogonal. 
Our contribution is to obtain a \emph{non-stationary} cost-to-go
function and its (sub)gradient for a finite-horizon problem using forward and
backward computations that scale efficiently with the size of the state space.
On the other hand, the results of~\cite{Ziebart2008MaxEnt} provide
a \emph{stationary} cost-to-go function and its gradient for an infinite horizon
problem.
The maximum entropy formulation of the stationary policy is a well grounded property 
of using a soft version of the Bellman update, which can explicitly model the 
suboptimality of expert trajectories.
However, we can show the benefits of our approach without including the maximum entropy
formulation and will leave it as future work.




==> tex/CostRepresentation.tex <==
\section{Cost Function Representation}
\label{sec:cost_representation}
% Map parameters
\newcommand{\tm}{\vec{\psi}}
% Map parameter at m-th ray
\newcommand{\tmm}{\tm_m}
% Map parameter k-th entry at m-th ray
\newcommand{\tmmk}{\psi_m^k}
% Map parameter k-th entry at m-th ray
\newcommand{\tmmkp}{\psi_m^{k'}}
% Cost Parameters
\newcommand{\tc}{\vec{\phi}}


%\begin{figure}[t]
%  \centering
%  \def\svgwidth{0.9\linewidth}
%  \input{fig/CostNeuralNet.pdf_tex}
%  %\includegraphics[width=\linewidth]{fig/CostNeuralNet}
%  \caption{Neural network model of a cost function. A recurrent neural network, parameterized by $\tm$, takes in sequential observations $\vec{P}_{1:t}$ and outputs a latent map representation. A convolutional neural network, parameterized by $\tc$, extracts features from the map state to specify the cost $c_t$ at a given robot state-control pair $(\vec{x},\vec{u})$. The learnable parameters are $\vec{\theta} = \crl{\tm, \tc}$.}
%  \label{fig:cost_neural_net}
%\end{figure}


We propose a cost function representation with two components: a \emph{semantic map encoder} 
with parameters $\tm$ and a \emph{cost encoder} with parameters $\tc$. 
The model is differentiable by design, allowing its parameters to be optimized
by the subsequent planning algorithm described in Sec.~\ref{sec:cost_learning}. 

%The map encoder incrementally updates a hidden state $\vec{h}_t$ using the most 
%recent semantic lidar point cloud $\vec{P}_t$ obtained from robot state $\vec{x}_t$. 
%For example, a recurrent neural network (RNN)~\citep{Goodfellow-et-al-2016} with 
%parameters $\tm$ can convert the sequential input $(\vec{x}_{1:t},\vec{P}_{1:t})$ 
%into a fixed-sized hidden state $\vec{h}_{t+1}$:
%\begin{equation}
%\vec{h}_{t+1} = \textbf{RNN}(\vec{h}_t, \vec{x}_t, \vec{P}_t; \tm).
%\end{equation}

\subsection{Semantic Map Encoder}
We encode the semantic occupancy probability of different environment areas into 
a hidden state $\vec{h}_t$. 
In detail, we discretize $\mathcal{X}$ into $J$ cells and let 
$\vec{m} = \brl{m^1, \dots, m^J}^T \in \mathcal{K}^J$ 
be the random vector of true semantic labels over the cells. 
Since $\vec{m}$ is unknown to the robot, we maintain the semantic occupancy 
likelihood $\mathbb{P}(\vec{m} = \vec{k} | \vec{x}_{1:t}, \vec{P}_{1:t})$
where $\vec{k} = \brl{k^1, \dots, k^J}^T, k^j \in \mathcal{K}$, given the history 
of states $\vec{x}_{1:t}$ and observations $\vec{P}_{1:t}$. 
The representation complexity may be simplified significantly if one assumes 
independence among the map cells $m^j$:
\begin{equation}
\label{eq:semantic_posterior}
\mathbb{P}(\vec{m} = \vec{k} | \vec{x}_{1:t}, \vec{P}_{1:t}) = 
\prod_{j=1}^J \mathbb{P}(m^j = k^j | \vec{x}_{1:t}, \vec{P}_{1:t}) \;.
\end{equation}
Inspired by the binary occupancy grid mapping~\citep{Thrun2005PR,Hornung2013Octomap}, 
we extend the recurrent updates for the multi-class semantic probability of 
each cell $m^j$. 
We define the log-odds ratio of semantic classes associated with cell $m^j$ 
at time $t$ as $\vec{h}_{t,j} = \brl{h_{t,j}^0, \dots, h_{t,j}^K}^T$, 
and its recurrent Bayesian update as:
\begin{equation}
h_{t,j}^k \defeq \log \frac{\mathbb{P}(m^j = 
k | \vec{x}_{1:t}, \vec{P}_{1:t})}{\mathbb{P}(m^j = 0 | \vec{x}_{1:t}, \vec{P}_{1:t})}
\;\text{for}\; k \in \mathcal{K}, \;\;\;
h_{t+1,j}^k = h_{t,j}^k 
+ \log\frac{\mathbb{P}(\vec{P}_{t+1} | m^j = k, \vec{x}_{t+1})}
{\mathbb{P}(\vec{P}_{t+1} | m^j = 0, \vec{x}_{t+1})}.
\end{equation}
Note that by definition $h_{t,j}^0 = 0$ and the update increment is a log-odds 
observation model. 
The semantic class posterior can be recovered from the semantic log-odds 
ratio $\vec{h}_{t,j}$ via a softmax function 
$\mathbb{P}(m^j = k | \vec{x}_{1:t}, \vec{P}_{1:t}) = 
\sigma^k(\vec{h}_{t,j})$,
where $\sigma : \mathbb{R}^{K+1} \rightarrow \mathbb{R}^{K+1}$ 
satisfies the following properties
\begin{equation}
\label{eqn:softmax}
\sigma(\vec{z}) = \brl{\sigma^0(\vec{z}), \dots, \sigma^K(\vec{z})}^T, \;
\sigma^k(\vec{z}) = \frac{\exp{(z^k)}}{\sum_{k' \in \mathcal{K}} \exp{(z^{k'})}}, \;
\log \frac{\sigma^k(\vec{z})}{\sigma^{k'}(\vec{z})} = z^k - z^{k'}.
\end{equation}
%
%\begin{proof}\NA{This can be skipped or moved into an appendix. We will not have space for it.}
%\begin{align*}
%    &\mathbb{P}(m^j = k | \vec{x}_{1:t}, \vec{P}_{1:t}) = e^{h_{t,j}^k} \mathbb{P}(m^j = 0 | \vec{x}_{1:t}, \vec{P}_{1:t}) \;, \\
%    & \sum_{k\in\mathcal{K}} \mathbb{P}(m^j = k | \vec{x}_{1:t}, \vec{P}_{1:t}) = 1 \\
%    &\Rightarrow \sum_{k\in\mathcal{K}} e^{h_{t,j}^k} \mathbb{P}(m^j = 0 | \vec{x}_{1:t}, \vec{P}_{1:t}) = 1 \\
%    &\Rightarrow \mathbb{P}(m^j = 0 | \vec{x}_{1:t}, \vec{P}_{1:t}) = \frac{1}{\sum_{k\in\mathcal{K}} e^{h_{t,j}^k}}
%\end{align*}
%\end{proof}
%
To complete the recurrent semantic class design, we parameterize the log-odds observation model:
\begin{equation}
\log\frac{\mathbb{P}(\vec{P} | m^j = k, \vec{x})}
{\mathbb{P}(\vec{P} | m^j = 0, \vec{x})} = 
\log\frac{\mathbb{P}(m^j = k | \vec{x}, \vec{P})}
{\mathbb{P}(m^j = 0 | \vec{x}, \vec{P})} - h_{0,j}^k =
{g_j^k(\vec{x},\vec{P})} - h_{0,j}^k 
\end{equation}
where Bayes rule is used to represent it in terms of an inverse observation model $g_j^k(\vec{x},\vec{P})$ and a prior occupancy log-odds ratio $h_{0,j}^k$, whose value may depend on the environment (e.g., $\vec{h}_{0,j} = \vec{0}$ specifies a uniform prior over the semantic classes). Note that map cells $m^j$ outside of the sensor field of view at time $t$ are not affected by $\vec{P}_t$, in which case $\vec{g}_j(\vec{x}_t,\vec{P}_t) = \vec{h}_{0,j}$. 

%\subsubsection{No Raycasting}\TW{need to remove this}
%Raycasting for lidar measurements is not necessary when there is 
%little noise~\citep{Zhou2019FastPlanner}.
%Consider a point $(\vec{p}_m, \vec{y}_m)$ in the point cloud $\vec{P}$ that lies in the 
%cell $m^j$.
%We augment the semantic prediction vector $\vec{y}_m = \brl{y_m^0, y_m^1, \dots, y_m^K}^T$
%with an additional entry, $y_m^0 = 0$, for the ``free class''.
%The inverse observation function can be modeled as a softmax with parameters $\tmm$:
%\begin{equation}
%\label{eqn:inv_obs}
%\mathbb{P}(m^j=k | \vec{x}, (\vec{p}_m, \vec{y}_m)) = 
%\frac{\exp{(\tmmk y_m^k)}} {\sum_{k' \in \mathcal{K}} \exp{(\tmmkp y_m^{k'})}}
%\end{equation}
%and the log-odds update rule can be simplified as:
%\begin{equation}
%h_{t+1,j}^k = h_{t,j}^k + \tmmk y_m^k - h_{0,j}^k\;,
%\end{equation}


Now consider all cells $m^j$ that lie on the ray between robot state $\vec{x}$ and the
point $\vec{p}_m$. 
Let $d(\vec{x}, m^j)$ be the distance between the robot position and the center of mass
of the cell $m^j$.
The inverse observation function can be modeled as a softmax with parameters $\tmm$,
scaled by the distance, $\delta p_m = d(m^j, \vec{x}) - \norm{\vec{p}_m}_2$, 
which is truncated at a threshold $\epsilon$:
\begin{equation}
\mathbb{P}(m^j = k | \vec{x}, (\vec{p}_m, \vec{y}_m)) = \begin{cases}
\sigma^k(\tmm \vec{y}_m \delta p_m)
%\frac{\exp{(\tmmk y_m^k \delta p_m)}} 
%{\sum_{k' \in \mathcal{K}} \exp{(\tmmkp y_m^{k'} \delta p_m)}} 
& \text{if } \delta p_m \leq\epsilon\\
%\frac{\exp{(h_{0,j}^k)}} 
%{\sum_{k' \in \mathcal{K}} \exp{(h_{0,j}^{k'})}} 
\sigma^k(\vec{h}_{0,j})
& \text{if } \delta p_m > \epsilon
\end{cases} \;.
\end{equation}
Using~\eqref{eqn:softmax}, the log-odds inverse sensor model for cells $m^j$ along the ray
from $\vec{x}_t$ to $\vec{p}_m$ becomes:
\begin{equation}
\label{eq:simple_inverse_sensor_model}
g_j^k(\vec{x}_t, (\vec{p}_m, \vec{y}_m)) = \begin{cases}
\tmmk y_m^k \delta p_m 
& \text{if } \delta p_m \leq\epsilon\\
h_{0,j}^k 
& \text{if } \delta p_m > \epsilon
\end{cases} \;.
\end{equation}
This suggests that a more expressive multi-layer neural network may be used instead of the linear transformation $\tmm \vec{y}_m \delta p_m $ of the semantic probability and distance differential along the $m$-th ray:
\begin{equation}
\label{eq:inverse_sensor_model}
\vec{g}_j(\vec{x}_t, (\vec{p}_m, \vec{y}_m);\tmm) = \begin{cases}
\textbf{NN}(\vec{y}_m, \vec{p}_m, d(\vec{x}_t, m^j) ; \tmm) 
& \text{if } \delta p_m \leq\epsilon\\
\vec{h}_{0,j}
& \text{if } \delta p_m > \epsilon
\end{cases}
\end{equation}
In summary, the map encoder starts with prior log-odds $\vec{h}_{0}$, 
updates them recurrently via $\vec{h}_{t+1} = 
\vec{h}_{t} + \vec{g}(\vec{x}_t,\vec{P}_t; \tm) - \vec{h}_{0}$,
where the inverse sensor log-odds $\vec{g}_j(\vec{x}_t, (\vec{p}_m, \vec{y}_m) ;\tmm)$ is specified for the $j$-th cell along the $m$-th ray in~\eqref{eq:inverse_sensor_model}.
The semantic posterior in~\eqref{eq:semantic_posterior} is the softmax output of $\vec{h}_{t}$.

\subsection{Cost Encoder}
The cost encoder uses the semantic occupancy grid prosterior $\sigma(\vec{h}_t)$ to 
define the cost function estimate $c_t(\vec{x},\vec{u})$ at a given state-control 
pair $(\vec{x},\vec{u})$. 
A convolutional neural network (CNN)~\citep{Goodfellow-et-al-2016} with parameters 
$\tc$ can extract cost features from the environment map:
\begin{equation}
c_t(\vec{x},\vec{u}) = \textbf{CNN}(\vec{h}_t, \vec{x}, \vec{u}; \tc).
\end{equation}
We implement an encoder-decoder neural network architecture~\citep{Badrinarayanan2017Segnet} 
to parameterize the cost function from semantic class probabilities.

%This conceptual model, combining recurrent estimation of a hidden environment state, 
%followed by feature extraction to define the cost at $(\vec{x}, \vec{u})$ is 
%illustrated in Fig.~\ref{fig:cost_neural_net} (\TODO{cannot include this figure}). 
%The model is differentiable by design, allowing its parameters 
%$\vec{\theta} = \crl{\tm,\tc}$ to be optimized. 
%We propose an instantiation of this general model, specific to modeling occupancy 
%costs from depth measurements in robot navigation tasks.


==> tex/Experiment.tex <==
\section{Experiments}
\label{sec:experiments}



We evaluate our approach using the CARLA simulator~\citep{Dosovitskiy2017CARLA} (0.9.6),
which provides high-fidelity autonomous vehicle simulation in urban environments.
Demonstration data for training the cost function representation is collected from 
maps $\crl{Town01, Town02, Town03, Town04}$, while map $Town05$ is used for testing. 
$Town05$ is the largest map and includes different street layouts, junctions, 
and a freeway. 
In each map, we collect $100$ expert trajectories by running the autonomous navigation 
agent provided by the CARLA Python API. 
The expert finds the shortest path between two query points, while respecting 
traffic rules, such as staying on the road, and keeping in the current lane. 
Features not related to the experiment are disabled, including spawning 
other vehicles and pedestrians, and changing traffic signal. 
Each robot trajectory is discretized into a $128\times128$ grid of $1$ meter resolution.
The robot state $\vec{x}$ is the grid cell location while the control $\vec{u}$ takes the 
robot to one of its $8$ neighbor grid cells.
Trajectories that do not fit in the grid are discarded.

The ego vehicle is equipped with a lidar sensor that has $20$ meters 
maximum range and $360^{\circ}$ horizontal field of view.
The vertical field of view ranges from $0^{\circ}$ 
(facing forward) to $-40^{\circ}$ (facing down) with $10^{\circ}$ resolution. 
A total of $56000$ lidar rays is generated per scan $\vec{P}_t$
while each point measurement is returned only if it hits an obstacle.
The ego vehicle is also equipped with $4$ semantic segmentation cameras 
that display objects of 13 different classes in RGB images, 
including road, road line, sidewalk, vegetation, car, building, etc.
The $4$ cameras face front, left, right and rear, each capturing a $90^{\circ}$ 
horizontal field of view. 
The semantic label of each lidar point is retrieved from the semantic segmentation
image by projecting the lidar point in the camera's frame.

In our model, we simplify the raycasting step in 
Eqn.~\eqref{eq:simple_inverse_sensor_model} by only
updating the log-odds at the cell that contains the lidar point, 
and not for the cells in between the robot and the point. 
The A* algorithm is used to solve the DSP~\eqref{eqn:Q}, providing the optimal cost-to-go 
$Q^*_t(\vec{x},\vec{u})$ for $\vec{x} \in \text{CLOSED} \cup \text{OPEN}$ and a subgradient
of $\mathcal{L}(\vec{\theta})$ according to Prop.~\ref{prop:chain_rule}. 
We compare our model to two baseline algorithms:~\citet{Wulfmeier2016DeepMaxEnt} 
and~\citet{Wulfmeier2016DeepMaxEnt} + semantics.
 \citet{Wulfmeier2016DeepMaxEnt} use a neural network to learn the cost from
lidar point clouds without semantics.
The input to the neural network is a grid that stores the mean and variance of the 
points in each cell, as well as a binary indicator of cell visibility at any frame. 
We augment the grid features with the mode of the semantic labels in each cell 
to get the model \citet{Wulfmeier2016DeepMaxEnt}~+~semantics as a fair comparison with ours.
All neural networks are implemented in the PyTorch library~\citep{Paszke2019Pytorch} and
trained with the Adam optimizer~\citep{Kingma2014ADAM} until convergence.

\begin{figure*}[t]
\begin{tabular}{c c c c c}
    \toprule
    Model & \makecell{\textit{NLL}} & \makecell{\textit{Acc} (\%)} & \makecell{\textit{Traj. Succ. Rate} (\%)} & \makecell{\textit{MHD}} \\
    \midrule
    ~\cite{Wulfmeier2016DeepMaxEnt} & 0.595 & 86.1 & \textbf{92} & 4.521 \\
    \makecell{~\cite{Wulfmeier2016DeepMaxEnt} $+$ semantics} & 0.613 & 82.7 & 88 & 4.479 \\
    Ours & \textbf{0.446} & \textbf{90.5} & 91 & \textbf{3.036} \\
    \bottomrule
\end{tabular}
\caption{Test result from CARLA \textit{Town05} map. Best model for each evaluation metric is in bold.}
\label{fig:test_results}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/test_result.pdf}
    \caption{
    Example of a predicted trajectory in red at an intersection. 
    The groud truth semantic map, predicted semantic map and cost map at two time steps are shown. 
    Our model learns the sidewalk is costly to traverse.}
    \label{fig:map_cost}
\end{figure*}

The evaluation metrics include: 
negative log-likelihood (\textit{NLL}), control accuracy (\textit{Acc}),
trajectory success rate (\textit{Traj. Succ. Rate}) and Modified Hausdorff Distance 
(\textit{MHD}). 
%NLL is defined in Eqn~\ref{eq:loss} where the learned policy $\pi$ is evaluated 
%along all states $\vec{x}_t$ along the trajectory.
%\textit{NLL} and \textit{Acc} measure the negative log-likelihood and accuracy 
%of the learned policy along the expert trajectory with respect to the expert controls.
More precisely, given a test set 
$\mathcal{D}_{test} = \crl{(\vec{x}_{t,n},\vec{u}_{t,n}^*,\vec{P}_{t,n}, 
\vec{x}_{g,n})}_{t=1, n=1}^{T_n, N}$ and a learned policy $\pi$ with paramters $\vec{\theta}^*$, we define $\textit{NLL}(\mathcal{D}_{test}, \pi) = 
- \frac{1}{\sum_{n=1}^{N} T_n} \sum_{n=1, t=1}^{N, T_n} 
\log \pi_{t,n}(\vec{u}_{t,n}^* | \vec{x}_{t,n}; \vec{P}_{1:t,n}, \vec{\theta}^*) $
and 
$\textit{Acc}(\mathcal{D}_{test}, \pi) = \frac{1}{\sum_{n=1}^{N} T_n} \sum_{n=1, t=1}^{N, T_n}
\indicator_{\crl{\vec{u}_{t,n}^* = \argmax \pi_{t,n}(\cdot | \vec{x}_{t,n}; 
\vec{P}_{1:t,n}, \vec{\theta}^*)}}$.
\textit{Traj. Succ. Rate} records the success rate of the learned policy by 
iteratively rolling out its predicted controls.
A trajectory is regarded as success if it reaches the goal within twice the number of 
steps of the expert trajectory without hitting an obstacle.
\textit{MHD} compares the rolled out trajectory $\vec{\tau}_{L}$ by the learned policy 
and the expert trajectory $\vec{\tau}_E$ and is defined as:
$
\textit{MHD} (\vec{\tau}_{L}, \vec{\tau}_{E}) = \max{
\crl{ \frac{1}{T_L}\sum_{t=1}^{T_L} d(\vec{\tau}_{L}^t, \vec{\tau}_{E}),
\frac{1}{T_E}\sum_{t=1}^{T_E} d(\vec{\tau}_{E}^t, \vec{\tau}_{L}) }}
$
where $d(\vec{\tau}_{A}^t, \vec{\tau}_{B})$ measures the minimum Euclidean distance from
state $\vec{\tau}_{A}^t$ to any state in $\vec{\tau}_{B}$.

Fig.~\ref{fig:test_results} shows the performance of our model versus~\citet{Wulfmeier2016DeepMaxEnt}  and~\citet{Wulfmeier2016DeepMaxEnt} + semantics
using the metrics described above. 
Ours learns to generate policy that is closest to the expert in new environments by
scoring best in \textit{NLL} and \textit{Acc}. 
The predicted trajectory is also closest to the expert by achieving the minimum \textit{MHD}.
The results demonstrate that the semantic map encoder captures more geometric as well as 
semantic information so that the cost function can be optimized and generate trajectories 
which match the expert behaviors.
We notice that simply taking the mode of the semantic labels in each grid cell degrades the 
performance of \citet{Wulfmeier2016DeepMaxEnt}.
We conjecture that taking the mode is a deterministic assignment, which could 
provide conflicting semantic information, while our model endorses a probabilistic semantic 
map encoder with Bayesian updates to avoid information loss.
For example, a cell with more road points than sidewalk points is assigned as road 
even though the expert would not traverse such cell.
Fig.~\ref{fig:map_cost} shows an example of the predicted trajectory at an intersection.
The semantic map visualizes the class of highest probability at each cell, 
which mostly reflects the ground truth.
The cost map identifies regions of high cost are on the sidewalk.


==> tex/RelatedWork.tex <==
\section{Related Work}
\label{sec:related_work}

%\begin{table}
%  \scriptsize
%  \centering
%  \begin{tabular}{lllll}
%    \toprule
%    $\downarrow$Reference \textbackslash Feature $\rightarrow$ & POE & PBB & DNN & CfG 
%    \\
%    \midrule
%    ~\cite{Tamar2016VIN} & \xmark & \xmark & \cmark & \xmark\\
%    ~\cite{Gupta2017CMP} & \cmark & \xmark & \cmark & \xmark\\
%    ~\cite{Ziebart2008MaxEnt} & \xmark & \xmark & \xmark & \cmark
%    \\
%    ~\cite{Ratliff2006MMP} & \xmark & \cmark & \xmark & \cmark
%    \\
%    ~\cite{Karkus2019DAN} & \cmark$^\dagger$ & \xmark & \cmark & \xmark
%    \\
%    Ours & \cmark & \cmark & \cmark & \cmark
%    \\
%    \bottomrule
%  \end{tabular}
%  \caption{Comparison with closely related work based on the use of Partially Observable Environments (POE),
%    Partial Bellman Backups (PBB), Deep Neural Network (DNN) representation, and Closed-form Gradients (CfG). PBB refers to computing and differentiating values over a subset of promising states as opposed to the whole state space. $^\dagger$~\cite{Karkus2019DAN} works with uncertainty only on the robot or furniture location, while the main environment structure is known.}
%    %$^*$ MaxEntIRL~\cite{Ziebart_MaxEnt08} is not able to take the full advantage of the closed-form gradient because they still have to perform full dynamic programming updates to compute gradient through the planning algorithms owing to the use of stochastic policy.
%  \label{tab:related-work}
%\end{table}

% Semantic mapping
Perceptions with semantic labels provide rich information about the relationship 
between object entities and the spatial environment. 
Various semantic segmentation techniques using deep neural networks are capable of 
predicting semantic labels of pixels in an RGB 
image~\citep{Papandreou2015WeakSemSeg,Badrinarayanan2017Segnet, Chen2018EncoderSemSeg} 
or a point cloud by projecting it onto a 2D spherical depth 
image~\citep{Wu2018SqueezeSeg, Dohan2015LidarSemSeg}.
Map representations that integrate such semantic information can facilitate 
planning in robot navigation.
~\citet{Sengupta2012SemMap, Lu2019MonoSemMap} show that dense 2D semantic maps can 
be generated from RGB images while \citet{Gan2019Bayesian, Sun2018ReccOctoMap} 
generalize the binary occupancy grid 
mapping~\citep{Hornung2013Octomap} to multi-class semantic mapping in 3D
where new observations can be incorporated incrementally using Bayesian inference 
or recurrent neural networks~\citep{Goodfellow-et-al-2016}. 
Post-processing optimization can be applied to enhance spatial smoothness and 
continuity of infering semantic probabilities. 
In this work, our model parameterizes the cost as a nonlinear function of 
such semantic mapping features to explain the expert bahaviors from its observation sequence.


% IRL
Learning a cost function from demonstrations requires a control policy that is 
differentiable with respect to the cost parameters. 
Computing such derivatives has been addressed by several sucessful IRL approaches~\citep{Neu2012Apprenticeship, Ratliff2006MMP, Ziebart2008MaxEnt}. 
Early works assume that the cost is linear in the feature vector and aim at matching the 
feature expectation between the learned policy and the expert policy. 
For example,~\citet{Ratliff2006MMP} propose to compute subgradients~\citep{Shor2012Subgradient}
of planning algorithms so that expected reward of expert policy is better than 
any other policies by a margin. 
\citet{Ziebart2008MaxEnt} develop a dynamic programming planning algorithm to maximize the 
likelihood of observed expert data and learn a policy of maximum entropy distribution.
Value iteration networks (VIN)~\citep{Tamar2016VIN} show that the value 
iteration algorithm \citep{Bertsekas1995OC} can be approximated by a series of 
convolution and maxpooling layers, allowing automatic differentiation to learn 
the cost function end-to-end. 

% mapping and irl
A series of recent works addresses IRL under partial observability. 
~\citet{Karkus2019DAN} formulate the IRL problem as a POMDP~\citep{Astrom1965POMDP}, 
including the robot pose and environment map in the state.
Since a na\"ive representation of the occupancy distribution may require
exponential memory in the map size, the authors assume partial knowledge of the
environment (the structure of a building is known but the furniture placement is
not).
Various works~\citep{Levine2011Nonlinear, Wulfmeier2016DeepMaxEnt, Song2019IRL} extend 
the one by \citet{Ziebart2008MaxEnt} and learn the cost as a nonlinear function in terms of
the feature vector using Gaussian processes~\citep{Rasmussen2003GP} or deep neural networks.
The cost function is learned offline provided with the full observation sequence along a
trajectory while we require an online planner that has access to only the observations 
so far at each step in a trajectory. 
\citet{Gupta2017CMP} propose to decompose visual navigation into two separate stages:
mapping the environment from first-person RGB images and planning through the constructed 
map with VIN~\citep{Tamar2016VIN}. 
Our model also seperates the two stages explicitly. 
In addition, we integrate semantic information to obtain a richer map representation and 
learn the cost parameterization with efficient Bellman backups and closed-form gradients. 


